TRUST: Test-Time Refinement using Uncertainty-Guided SSM Traverses

State Space Models (SSMs) have emerged as efficient alternatives to Vision Transformers (ViTs), with VMamba standing out as a pioneering architecture designed for vision tasks. However, their generalization performance degrades significantly under distribution shifts. To address this limitation, we propose TRUST (Test-Time Refinement using Uncertainty-Guided SSM Traverses), a novel test-time adaptation (TTA) method that leverages diverse traversal permutations to generate multiple causal perspectives of the input image. Model predictions serve as pseudo-labels to guide updates of the Mamba-specific parameters, and the adapted weights are averaged to integrate the learned information across traversal scans. Altogether, TRUST is the first approach that explicitly leverages the unique architectural properties of SSMs for adaptation. Experiments on seven benchmarks show that TRUST consistently improves robustness and outperforms existing TTA methods.

==> Backup/math_commands.tex <==
\usepackage{amssymb,amsmath,amsthm,amsfonts,bm}
\usepackage{multirow}
\usepackage{booktabs}
\usepackage{tabularx}
\usepackage[table]{xcolor}
%\usepackage{epsfig}
\usepackage{pgf}
\usepackage{cancel}
\usepackage{wrapfig}
\usepackage{microtype}
\usepackage{xspace}
\usepackage{pifont}
\usepackage{scalerel}
\usepackage{graphicx}
\usepackage{tikz}
\usepackage{mathtools}
\usepackage{svg}
\usepackage{hyperref}
\usepackage{dsfont}
\usepackage{enumitem}

\newcommand{\dorowcolors}{\rowcolors{2}{gray!15}{white}}
\definecolor{cliptta_color}{rgb}{1, 0.97, 0.92}
\definecolor{lightgray}{rgb}{0.95, 0.95, 0.95}
\definecolor{BrickRed}{rgb}{0.8, 0.25, 0.33}
\definecolor{OliveGreen}{rgb}{0.33, 0.42, 0.18}

\newcommand{\mypar}[1]{\vspace{3pt}\noindent\textbf{#1~}}
\newcommand{\CLIPTTA}{C\textsc{lip}TTA\xspace}
\newcommand{\CLIPTTAb}{\textbf{C\textsc{lip}TTA}\xspace}

\newcommand{\theHalgorithm}{\arabic{algorithm}}
\newcommand\wh[1]{\hstretch{1.25}{\hat{\hstretch{.8}{#1}}}}
\newcolumntype{Y}{>{\centering\arraybackslash}X}

\newcommand{\eg}{\emph{e.g., }}
\newcommand{\ie}{\emph{i.e., }}

\newcommand{\sota}{\emph{state-of-the-art} }

% Mathematical caligraphy/sets
\newcommand{\mX}{\mathcal{X}}
\newcommand{\mY}{\mathcal{Y}}
\newcommand{\mZ}{\mathcal{Z}}
\newcommand{\mD}{\mathcal{D}}
\newcommand{\mP}{\mathcal{P}}

% Matrices and vectors
\newcommand{\XX}{\mathbf{X}}
\newcommand{\ZZ}{\mathbf{Z}}
\newcommand{\YY}{\mathbf{Y}}
\newcommand{\TT}{\mathbf{T}}
\newcommand{\QQ}{\mathbf{Q}}
\newcommand{\xx}{\mathbf{x}}
\newcommand{\yy}{\mathbf{y}}
\newcommand{\zz}{\mathbf{z}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}
\def\vt{{\bm{t}}}
\def\ve{{\bm{e}}}
%\def\vvk{{\bm{k}}
%\def\vvq{{\bm{q}}
\newcommand{\tr}[1]{{#1^{\top}}}

\newcommand{\boldEps}{\boldsymbol{\epsilon}}

%Elements of vectors
\def\evp{{p}}

%Random vectors
\def\rvz{{\mathbf{z}}}

% Important sets
\newcommand{\sR}{\mathbb{R}}

% Losses
\newcommand{\Lce}{\mathcal{L}_{\text{ce}}}
\newcommand{\Lim}{\mathcal{L}_{\text{IM}}}
\newcommand{\Lcls}{\mathcal{L}_{\text{cls}}}
\newcommand{\Lssl}{\mathcal{L}_{\text{ssl}}}
\newcommand{\Luns}{\mathcal{L}_{\text{uns}}}
\newcommand{\Lttt}{\mathcal{L}_{\text{ttt}}}
\newcommand{\Laux}{\mathcal{L}_{\text{aux}}}
\newcommand{\Lcont}{\mathcal{L}_{\text{cont}}}
\newcommand{\Lscont}{\mathcal{L}_{\text{s-cont}}}
\newcommand{\Loss}{\mathcal{L}}
\newcommand{\mr}[1]{\mathrm{#1}}
\newcommand{\Ls}{\mathcal{L}}

% Math symbols
\newcommand{\pphi}{\boldsymbol{\phi}}

% Statistics
\newcommand{\ppm}{\,\scriptsize$\pm$}

%Operators
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

%Theorems
\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{property}[theorem]{Property}
\theoremstyle{definition}
%\newtheorem{definition}[theorem]{Definition}
\newtheorem{assumption}[theorem]{Assumption}
\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}

==> Backup/sec/1_intro.tex <==
\section{Introduction}

% cnn and vit with their limitation / ssm as alternative / challenges of ssm in distribution shift
The field of visual representation learning has advanced rapidly due to the ability of deep neural networks to extract rich and generalizable features. \glspl{cnn} \cite{simonyan2014very, he2016deep, huang2017densely, tan2019efficientnet, liu2022convnet} excel at modeling local patterns through strong inductive biases but struggle with global context. \glspl{vit} \cite{dosovitskiy2020image, liu2021swin, zhang2023hivit, touvron2021training} address this using self-attention mechanism, although with a higher computational cost. More recently, \glspl{ssm} \cite{gu2021efficiently, fu2022hungry, smith2022simplified} emerged as a scalable alternative, providing global receptive fields with linear complexity. Despite their efficiency, the performance of \glspl{ssm} degrade under distribution shift due to violations of the \gls{iid} assumption, which is often disrupted in real-world settings. While generalization strategies are well-developed for \glspl{cnn} and \glspl{vit}, vision-specific strategies for \glspl{ssm} are still lacking.

% VMamba and its challenges in distribution shift
In this work, we focus on \emph{VMamba} \cite{liu2024vmamba}, a vision-adapted variant of the Mamba architecture~\cite{gu2023mamba}, designed for sequential visual processing. VMamba introduces \gls{ss2d}, a four-way traversal mechanism that scans image patches along predefined spatial directions. However, this directional processing introduces a strong inductive bias by aligning internal representations with fixed traversal paths \cite{dastani2025spectral}, which can hinder generalization under distribution shifts. Additionally, VMamba's hidden states store historical context over the traversal sequence. When exposed to unseen domains, this context may accumulate domain-specific artifacts, leading to amplified bias during propagation and ultimately degrading generalization~\cite{dgmamba}.

% our solution
To address these challenges, we propose \gls{trust}, a novel \gls{tta} strategy specifically designed for \glspl{ssm} that leverages VMamba's internal traversal mechanism. As illustrated in Figure~\ref{main_figure} offline mode, different traversal permutations result in varying prediction entropy levels, revealing the model's sensitivity to causal ordering. \gls{trust} systematically generates multiple traversal permutations by reordering the four directional scans, exposing the model to diverse causal perspectives of the same input. At test time, we compute the entropy of predictions from each permutation and select the ones with minimal entropy (uncertainty), which are empirically associated with more stable and domain-robust hidden states. 

Inspired by prior work on flat minima and weight averaging \cite{keskar2016large, cha2021swad}, our method aggregates outputs from different traversal permutations to implicitly explore a broader and flatter region of the loss landscape. Each permutation activates a distinct computational pathway through the model, effectively sampling different local minima. Selecting the top-k traversal permutations with the lowest predictive entropy and computing a weighted average of their model parameters, mitigates the impact of noisy or uncertain predictions. This enhances generalization without requiring source data or model retraining.

% summary
%In summary, we propose \gls{trust}, a test-time adaptation strategy tailored to VMamba's four-directional traversal mechanism to improve generalization under distribution shift. 
%Our approach mitigates the inductive bias introduced by fixed traversal directions and reduces the accumulation of domain-specific artifacts in hidden states. By permuting traversal directions and averaging model weights from the most confident paths, our method leverages directional diversity to enable robustness. Unlike prior \gls{tta} methods that depend on data augmentation or auxiliary models, \gls{trust} is inherently architecture-aware. 

Our main contributions are summarized as follows:

\begin{itemize}
    \item We propose \gls{trust}, the first \gls{tta} approach specifically designed for Mamba-based vision models. Unlike prior methods that depend on data augmentation or auxiliary models, our approach exploits the internal traversal dynamics of VMamba to improve generalization under distribution shift.
    \item \gls{trust} introduces a novel weighted averaging strategy to promote robustness, which permutes traversal directions and averages model weights from the most confident paths. 
    %Our approach mitigates the inductive bias introduced by fixed traversal directions and reduces the accumulation of domain-specific artifacts in hidden states.     
    %aimed at improving generalization under distribution shift.
    %\item Our approach uniquely exploits the \textbf{internal traversal dynamics} of VMamba to perform \textbf{informed weighted averaging} over multiple causal views.
    % , in contrast to prior work that relies on data augmentations or handcrafted templates.
    %\item Unlike prior \gls{tta} methods that depend on data augmentation or auxiliary models, \gls{trust} is inherently architecture-aware and  
    \item We validate our method on \textbf{seven standard benchmarks}, where it consistently outperforms existing \gls{tta} methods, establishing new state-of-the-art results.
\end{itemize}

==> Backup/sec/2_relatedwork.tex <==
\vspace{-10pt}
\section{Related Work}
\vspace{-5pt}

\textbf{\acrfull{tta}} is a paradigm of Domain Adaptation (DA)~\cite{shot} that intends to enhance a model's generalization capabilities in real time during deployment. Specifically, a pretrained model is adapted to incoming data streams (\ie batches) independently, without requiring label supervision nor having access to source data. As pioneering approach, TENT~\cite{tent} minimizes prediction entropy as adaptation objective, based on the principle that distribution shifts in the target domain reduce the model's confidence in its predictions.
%This framework of entropy minimization has been thoroughly investigated as a natural continuation of the standard supervised pretraining based on cross-entropy, although it does not necessarily exploit the inherent working mechanisms of any model in particular. 
Examples of TENT-based approaches include using confidence thresholds for sample selection before adaptation~\cite{eta,ostta}, minimizing the sharpness of the entropy loss~\cite{sar}, using class balanced memory queues for better adaptation sampling~\cite{rotta}, and meta-learning the entropy loss~\cite{conjugate}, among other alternatives~\cite{sotta,stamp,unient}. 
Several adaptation strategies that do not depend on entropy minimization have also been proposed in the literature, such as contrastive learning~\cite{cotta,adacontrast}, Laplacian optimization~\cite{lame,program}, and prototype-based pseudo-labeling~\cite{tast}. While flexible, these techniques do not capitalize on the unique properties of specific architectures such as VMamba. 

\textbf{Architecture-specific \gls{tta}}. Recent advancements in \gls{tta} have introduced a variety of model-specific strategies. Among those, FOA~\cite{foa} loosely adheres to ViTs by incorporating the gradient-free learning of additional prompts in the form of token embeddings. For Vision-language Models (VLM)~\cite{tpt,tda,watt,clipartt}, recent strategies incorporate text information as an auxiliary tool for adaptation. Examples include prompt learning via entropy minimization~\cite{tpt}, positive and negative caching with text-based pseudolabels~\cite{tda}, transductive adaptation using conformal pseudocaptions~\cite{clipartt}, and weight averaging across text templates~\cite{watt}. SSM-oriented \gls{tta} has also been explored to a smaller extent. In a recent work, STAD~\cite{stad} uses Markov processes to learn time-varying prototypes for classifying examples during inference. Unlike our approach, which adapts each VMamba block by averaging the weights from confident paths, this previous method only adapts the model's classification head.

\textbf{Weight averaging for robust adaptation.}Initially introduced in the context of Domain Generalization (DG)~\cite{metadg,mixstyle,fds}, weight averaging has gained popularity as an effective technique for enhancing model robustness to domain shifts~\cite{swa,swad}. Notably, methods like SWAD~\cite{swad} aim to identify flat minima in the loss landscape by minimizing loss fluctuations across diverse inputs. This is often accomplished by averaging the weights of models trained on different image augmentations. While similar ideas have been adopted in the \gls{tta} literature~\cite{sar,watt}, they typically rely on explicit input diversification, which introduces additional computational overhead. In contrast, our approach leverages the intrinsic diversity of SSM-based traversals to induce variation in the model's weights, without requiring external data augmentations.

\begin{figure}[t]
    \centering
    % \includegraphics[width=\linewidth]{images/ss2d.pdf}
    \includegraphics[trim=0 680 0 0, clip, width=\textwidth]{images/ss2d.pdf}
    \vspace{-15pt}
    \caption{}
    \label{main_figure}
\end{figure}

==> Backup/sec/3_method.tex <==
\section{Method}

Section~\ref{preliminary} introduces key concepts in \gls{tta} and \gls{ssm}, laying the groundwork for our approach. In Section~\ref{traverse}, we propose traversal permutations to address domain shifts, followed by a weight averaging strategy in Section~\ref{wa} for robust and efficient inference. An overview of the full method is provided in Figure~\ref{main_figure}.

\subsection{Preliminaries}\label{preliminary}

\mypar{\acrfull{tta} in image classification.} Consider a classification model composed of a feature processor $f_\theta$, parameterized by $\theta$, and a classifier $h_\phi$ parameterized by $\phi$. The model is pre-trained on a source dataset $\mathcal{D}_s = \{(\XX_j, y_j)\}_{j=1}^{N_s}$ consisting of images $\XX_j$ and corresponding labels $y_j$ ($F_s: \mathcal{X}_s \rightarrow \mathcal{Y}_s$). Training on $\mathcal{D}_s$ is performed using a supervised loss $\mathcal{L}_{\text{train}}$ (typically cross-entropy). At test-time, the model is exposed to a target dataset $\mathcal{D}_t = \{\XX_i\}_{i=1}^{N_t}$, which lacks labels and follows a different distribution, giving rise to the map $F_t: \mathcal{X}_t \rightarrow \mathcal{Y}_t$. Although the source and target datasets share the same label space ($\mathcal{Y}_s = \mathcal{Y}_t$), their joint distribution differ, \ie $P(\mathcal{X}_s,\mathcal{Y}_s) \neq P(\mathcal{X}_t, \mathcal{Y}_t)$. Such difference is referred to as \emph{covariate domain shift}~\cite{lame}.

\mypar{\acrfull{ssm} formulation.} \gls{ssm}-based models \cite{gu2021efficiently, mamba} map a 1D input sequence $\xx(t) \in \Real$ to an output $\yy(t) \in \Real$ through a learnable hidden state $\hh(t) \in \Real^N$, governed by a linear dynamical system:
\begin{equation}
    \hh(t) = \AAA \hh(t\!-\!1) + \BB \xx(t), \quad \yy(t) = \CC \hh(t), \label{mamba}
\end{equation}
where $\AAA \in \mathbb{R}^{N \times N}$, $\BB \in \mathbb{R}^{N \times 1}$, and $\CC \in \mathbb{R}^{1 \times N}$ are learnable parameters. To integrate this formulation into deep learning, it is discretized using the zero-order hold (ZOH) method with step size $\Delta \in \mathbb{R}$, resulting in the discrete recurrence:
\begin{equation}
    \hh(t) = \overline{\AAA} \hh(t-1) + \overline{\BB} \xx(t), \quad \yy(t) = \CC \hh(t),  \quad \texttt{where} \quad \overline{\AAA} = \exp(\Delta \AAA), \quad \overline{\BB} \approx \Delta \BB.
\end{equation}
Unrolling this recurrence over time yields a 1D convolution with kernel $\overline{\KK} \in \mathbb{R}^L$, where $L \in \mathbb{N}$ denotes the kernel length. This form enables efficient parallel computation during training.
\begin{equation}
    \yy = \xx \odot \overline{\KK}, \quad \overline{\KK} = \left( \CC \overline{\BB}, \CC \overline{\AAA} \overline{\BB}, \ldots, \CC \overline{\AAA}^{L-1} \overline{\BB} \right).
\end{equation}
\mypar{SS2D for 2D visual processing.} To extend 1D state-space models to visual data, VMamba introduces the \gls{ss2d} module, which reshapes an input image $\XX \in \mathbb{R}^{H \times W \times C}$ into a sequence of $T$ non-overlapping patches $\{\xx_t\}_{t=1}^{T}$. These patches are traversed in a predefined causal order determined by one of four canonical directions using the Cross-Scan module:  left-to-right ($a$), top-to-bottom ($b$),  right-to-left ($c$), and bottom-to-top ($d$). For each direction, the patch sequence is processed recurrently by a shared, discretized 1D \gls{ssm}, ensuring causality and directional consistency. The outputs from all four directional passes are then aggregated using the Cross-Merge module.

\subsection{Traversal Permutation}\label{traverse}

% VMamba's directional traversal mechanism introduces two critical challenges when faced with distribution shift. First, the use of fixed traversal paths imposes a strong inductive bias, aligning internal representations with specific scan orders and thereby restricting generalization. Second, the model's hidden states retain accumulated historical context along the traversal sequence. This context can encode domain-specific artifacts, which may be amplified during propagation, ultimately degrading the model's performance on unseen domains.

To address the challenges posed by distribution shifts, we propose a \gls{tta} strategy that leverages VMamba's intrinsic directional traversal mechanism. We define a set of traversal permutations \begin{equation} 
\mathcal{P} = \{\pi_1, \pi_2 \dots, \pi_N\},
\end{equation} 
where each $\pi_i$ represents a unique ordering of the four canonical scan directions, with $\pi_1 = \{(a), (b), (c), (d)\}$ corresponds to the original ordering used in VMamba. We assess the predictive confidence of the model under each traversal permutation $\pi_i \in \mathcal{P}$ by computing the \textit{Shannon entropy} of its output distribution. Permutations are then ranked in ascending order of entropy, and the top-$K$ permutations with the lowest entropy are selected (Figure~\ref{main_figure} offline mode): 
\begin{equation} 
\mathcal{P}_\texttt{selected} = \{\pi_{i_1}, \pi_{i_2}, \dots, \pi_{i_K} \}. 
\end{equation} 

During the adaptation phase, for each selected permutation $\pi_{i_k}$, $k=1,\ldots,K$, the input is processed according to the corresponding traversal order, and pseudo-labels $\hat{y}^{(i_k)}$ are assigned by taking the class with maximum predicted probability. The model's parameters are then updated to minimize the cross-entropy loss between the model's prediction and the corresponding pseudo-label. Here, the expectation $\mathbb{E}$ is taken over the distribution of $\mathcal{P}$. After optimization, the adapted parameter set $\theta^{(i_k)}$ is cached, allowing a subsequent ensemble-based aggregation at inference: 
\begin{equation} 
\boldsymbol{\theta}^{(i_k)} = \arg\min_{\boldsymbol{\theta}} \, \mathbb{E}\left[ \mathrm{CE} \left( \hat{y}^{(i_k)}, \, f_{\boldsymbol{\theta}}(\XX_{\pi_{i_k}}) \right) \right].
\end{equation}

Our method processes the same image through multiple directional permutations, enabling VMamba to exploit complementary causal views of the input. These distinct trajectories expose the model to both global consistency (identical token set) and local variation (different hidden‑state evolutions), which empirical studies link to flatter minima and stronger \gls{ood} generalization \cite{swad}. Crucially, re‑ordering prevents domain‑specific artifacts from always entering the recurrence at the same time step. 
If an artefact $\boldsymbol{\varepsilon}$ is embedded in a corrupted patch $\xx_{t_{\boldsymbol{\varepsilon}}}$, then under the default traversal $\pi_1$, this patch always appears at time step $t = t_{\boldsymbol{\varepsilon}}$ in the processing sequence. The hidden state update at that step becomes:
\begin{equation}
    \hh^{(1)}(t_{\boldsymbol{\varepsilon}}) = f\left(\hh^{(1)}(t_{\boldsymbol{\varepsilon}} - 1),\, \xx_{t_{\boldsymbol{\varepsilon}}} + \boldsymbol{\varepsilon} \right).
\end{equation}

Since the hidden state $\hh(t)$ is recurrent and accumulates over time, injecting $\boldsymbol{\varepsilon}$ early in the sequence allows its influence to propagate through many subsequent updates. Therefore, the impact of the artefact depends heavily on the position of $t_{\boldsymbol{\varepsilon}}$ within the sequence.

In our method, we apply a traversal permutation $\pi_i$, which changes the order in which patches are processed. Under $\pi_i$, the corrupted patch $\xx_{t_{\boldsymbol{\varepsilon}}}$ appears at time step $t = \pi_i(t_{\boldsymbol{\varepsilon}})$, leading to the updated hidden state:
\begin{equation}
    \hh^{(i)}\left(\pi_i(t_{\boldsymbol{\varepsilon}})\right) = f\left(\hh^{(i)}\left(\pi_i(t_{\boldsymbol{\varepsilon}}) - 1\right),\, \xx_{t_{\boldsymbol{\varepsilon}}} + \boldsymbol{\varepsilon} \right).
\end{equation}

Across different permutations, the corrupted patch enters the sequence at varying time steps. This shifts the artefact’s effect to different hidden states, breaking its consistent influence pattern. During test-time adaptation, these variations allow the model to learn diverse responses, and the subsequent entropy-weighted model averaging helps suppress artefact-induced bias.


\subsection{Leveraging Traversal Permutations through Weight Averaging}\label{wa}

To improve both stability and generalization under distribution shifts, we aggregate the adapted models obtained from the top-$K$ traversal permutations. During evaluation phase, we utilize the averaged weights $\bar{\theta}$ and we evaluate the model using the default traversal path $\pi_1$. This results in a single, consolidated model that captures the benefits of multi-directional adaptation. 
\begin{equation}
\bar{\theta} = \frac{1}{K} \sum_{k=1}^{K} \theta^{(i_k)}
\end{equation}

This simple yet effective averaging strategy draws inspiration from the notion of \textit{flat minima} in the loss landscape \cite{swa,swad}, where parameter configurations that lie in flat regions tend to exhibit greater generalization and robustness to perturbations. Weight averaging encourages convergence to a region in parameter space with low curvature, thereby reducing sensitivity to input variations and improving performance under distribution shifts. In this setting, each $\theta^{(i_k)}$ represents a model adapted under a distinct traversal bias. Averaging over these directions allows us to approximate a solution residing in the intersection of several flat regions, yielding a more stable and transferable model.

Unlike traditional \gls{tta} approaches that rely on data augmentation, external supervision, or access to source data, our approach exploits VMamba's inherent architectural bias, its directional traversal mechanism, to generate diverse causal views of the same input. By averaging model weights across multiple traversal permutations, we achieve improved generalization through flatter minima in the loss landscape and enhanced stability by mitigating noise from individual adaptation paths.

\textcolor{red}{WE HAVE TO ADD LOSS LAND SCAPE FIGURE FOR OUR METHOD!}

% The averaging mechanism offers two key advantages: (1) Improved Generalization via Flat Minima: By combining weights from multiple traversal-permutation models, the averaged solution is more likely to reside in a low-curvature region of the loss landscape. Such regions are associated with stable performance under varying data conditions, thereby reducing susceptibility to traversal-specific overfitting. (2) Stability through Noise Mitigation: Aggregating parameters across different adaptation paths reduces the influence of noise or unreliable updates that may occur due to corrupted inputs or pseudo-label errors. The resulting model is more resilient and consistent across diverse test-time scenarios.



==> Backup/sec/4_experiments.tex <==
\section{Experiments}
In this section, we present a comprehensive evaluation of our proposed method across seven benchmark datasets: CIFAR10-C, CIFAR100-C, ImageNet-C, ImageNet-Sketch, ImageNet-V2, ImageNet-R, and PACS. These datasets span a wide spectrum of real-world challenges, including diverse corruption types, domain shifts, and distributional variations. By conducting experiments on this diverse set, we aim to rigorously assess the robustness and generalization ability of our approach under both synthetic and natural distribution shifts. The results highlight the effectiveness of our method in handling a broad range of complex scenarios.

\subsection{Datasets}
We evaluate the performance and generalization capability of our method across a broad range of \gls{tta} benchmarks, covering both corruption-based robustness and domain generalization. To assess robustness to common corruptions, we evaluate on CIFAR10-C, CIFAR100-C, and ImageNet-C \cite{corruption}. These benchmarks apply 15 algorithmically generated corruption types, including noise, blur, weather effects, and digital artifacts, at five severity levels to the clean CIFAR10, CIFAR100, and ImageNet datasets. CIFAR10-C features $10$ coarse-grained classes, while CIFAR100-C includes $100$ fine-grained categories, offering a more challenging evaluation. ImageNet-C extends these corruptions to the large-scale ImageNet dataset with $1000$ categories, enabling a systematic analysis of model degradation under real-world visual distortions.

To evaluate generalization across domain shifts, we consider PACS \cite{pacs}, ImageNet-Sketch (ImageNet-S) \cite{sketch}, ImageNet-V2 \cite{v2}, and ImageNet-Rendition (ImageNet-R) \cite{R}. PACS comprises four visually distinct domains (Photo, Art Painting, Cartoon, and Sketch), with a shared label space of seven classes. We follow the standard leave-one-domain-out evaluation protocol. ImageNet-S consists of sketch-style representations of ImageNet classes, testing generalization to abstract and minimalist visual forms. ImageNet-V2 offers a cleaner and independently collected test set from the same distribution as ImageNet. ImageNet-R contains $30,000$ images across $200$ ImageNet classes, covering a wide range of artistic renditions including paintings, cartoons, graffiti, embroidery, and video game graphics. It presents a challenging benchmark for style-based distribution shifts. These datasets collectively enable a comprehensive evaluation of a model’s ability to adapt to unseen styles, abstractions, and distributions.

\begin{table*}[htbp]
\setlength\tabcolsep{4pt}
\centering
\resizebox{0.9\textwidth}{!}{
\small
\begin{tabular}{l|l|ccccccccccccccc|c}
\toprule
& Method & \rotatebox{90}{gaussian noise} & \rotatebox{90}{shot noise} & \rotatebox{90}{impulse noise} & \rotatebox{90}{defocus blur} & \rotatebox{90}{glass blur} & \rotatebox{90}{motion blur} & \rotatebox{90}{zoom blur} & \rotatebox{90}{frost} & \rotatebox{90}{snow} & \rotatebox{90}{fog} & \rotatebox{90}{brightness} & \rotatebox{90}{contrast} & \rotatebox{90}{elastic} & \rotatebox{90}{pixelate} & \rotatebox{90}{jpeg compression} & Mean \\
\midrule
\parbox[t]{4mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{CIFAR10-C}}} 
& Source only           & 46.8 & 48.4 & 45.0 & 73.5 & 52.6 & 73.0 & 78.7 & 71.8 & 75.8 & 77.3 & 85.7 & 69.6 & 63.7 & 67.9 & 59.0 & 65.9 \\
& ETA \cite{eta}        & 46.7 & 48.3 & 44.8 & 73.5 & 52.6 & 73.0 & 78.6 & 75.7 & 71.4 & 77.2 & 85.7 & 69.6 & 63.7 & 67.9 & 59.0 & 65.8 \\
& LAME \cite{lame}      & 46.7 & 48.3 & 44.8 & 73.5 & 52.6 & 73.0 & 78.6 & 71.8 & 75.8 & 77.2 & 85.7 & 69.6 & 63.7 & 67.9 & 59.0 & 65.9 \\
& SAR \cite{sar}        & 47.7 & 49.5 & 46.2 & 74.3 & 53.4 & 73.8 & 79.1 & 72.5 & 76.5 & 78.0 & 86.1 & 70.8 & 64.5 & 68.9 & 60.0 & 66.8 \\
\cmidrule{2-18}
& SHOT \cite{shot}      & 47.8 & 49.7 & 46.3 & 74.3 & 53.7 & 74.0 & 79.3 & 72.6 & 76.6 & 78.1 & 86.3 & 70.7 & 64.5 & 68.9 & 59.9 & 66.8 \\
& TENT \cite{tent}      & 47.3 & 49.2 & 45.8 & 74.2 & 53.1 & 73.7 & 79.1 & 72.2 & 76.3 & 77.9 & 86.1 & 70.4 & 64.3 & 68.7 & 59.6 & 66.5 \\
& \gls{trust} naive            & 58.9 & 61.8 & 62.0 & 79.8 & 60.9 & 79.1 & 82.6 & 80.5 & 81.8 & 83.6 & 88.8 & 81.8 & 70.3 & 75.1 & 66.0 & 74.2 \\
& \ccol \gls{trust}            & \ccol \textbf{63.1} & \ccol \textbf{67.8} & \ccol \textbf{70.3} & \ccol \textbf{81.0} & \ccol \textbf{64.5} & \ccol \textbf{81.4} & \ccol \textbf{85.0} & \ccol \textbf{83.2} & \ccol \textbf{85.4} & \ccol \textbf{85.8} & \ccol \textbf{90.1} & \ccol \textbf{85.7} & \ccol \textbf{72.1} & \ccol \textbf{79.1} & \ccol \textbf{68.6} & \ccol \textbf{77.5} \\
\midrule
\midrule
\parbox[t]{4mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{CIFAR100-C}}} 
& Source only           & 21.0 & 22.1 & 18.3 & 50.6 & 27.7 & 51.0 & 56.2 & 45.3 & 50.6 & 52.4 & 65.3 & 43.2 & 39.0 & 41.7 & 33.4 & 41.2 \\
& ETA \cite{eta}        & 21.2 & 22.3 & 18.7 & 50.8 & 27.8 & 51.2 & 56.3 & 45.4 & 50.8 & 52.7 & 65.5 & 43.5 & 39.2 & 42.0 & 33.7 & 41.4 \\
& LAME \cite{lame}      & 21.0 & 22.1 & 18.3 & 50.6 & 27.7 & 51.0 & 56.2 & 45.3 & 50.6 & 52.5 & 65.4 & 43.2 & 39.0 & 41.7 & 33.4 & 41.2 \\
& SAR \cite{sar}        & 21.9 & 22.8 & 19.3 & 51.1 & 28.2 & 51.5 & 56.7 & 46.4 & 51.4 & 53.1 & 65.8 & 44.2 & 39.9 & 42.8 & 34.2 & 41.9 \\
\cmidrule{2-18}
& SHOT \cite{shot}      & 21.9 & 22.9 & 19.1 & 51.4 & 28.3 & 51.8 & 56.8 & 46.3 & 51.4 & 53.3 & 66.0 & 44.2 & 39.8 & 42.7 & 34.3 & 42.0 \\
& TENT \cite{tent}      & 21.6 & 22.6 & 18.9 & 51.1 & 28.2 & 51.5 & 56.7 & 46.2 & 51.1 & 53.1 & 65.8 & 44.0 & 39.7 & 42.5 & 34.0 & 41.8 \\
& \gls{trust} naive            & 32.1 & 32.8 & 34.1 & 56.9 & 35.4 & 57.2 & 61.6 & 54.6 & 57.8 & 60.1 & 69.6 & 55.6 & 46.6 & 50.8 & 41.0 & 49.8 \\
& \ccol \gls{trust}            & \ccol \textbf{37.8} & \ccol \textbf{38.9} & \ccol \textbf{42.3} & \ccol \textbf{60.9} & \ccol \textbf{36.6} & \ccol \textbf{60.8} & \ccol \textbf{65.4} & \ccol \textbf{59.0} & \ccol \textbf{62.2} & \ccol \textbf{64.5} & \ccol \textbf{71.7} & \ccol \textbf{63.1} & \ccol \textbf{50.3} & \ccol \textbf{56.6} & \ccol \textbf{44.9} & \ccol \textbf{54.3} \\
\midrule
\midrule
\parbox[t]{4mm}{\multirow{7}{*}{\rotatebox[origin=c]{90}{ImageNet-C}}} 
& Source only           & 24.3 & 26.1 & 25.1 & 22.2 & 23.2 & 35.4 & 43.2 & 49.3 & 48.4 & 56.9 & 70.0 & 26.8 & 45.1 & 43.7 & 41.4 & 38.7 \\
& ETA \cite{eta}        & 26.4 & 28.4 & 27.2 & 23.5 & 24.6 & 37.2 & 45.1 & 50.8 & 51.0 & 58.8 & 70.6 & 29.1 & 47.7 & 46.9 & 45.0 & 40.8 \\
& LAME \cite{lame}      & 24.3 & 26.1 & 25.1 & 22.2 & 23.2 & 35.4 & 43.2 & 49.3 & 48.4 & 56.9 & 70.0 & 26.8 & 45.1 & 43.7 & 41.4 & 38.8 \\
& SAR \cite{sar}        & 26.5 & 29.2 & 28.0 & 24.5 & 25.3 & 37.4 & 45.3 & 51.0 & 51.7 & 59.0 & 70.5 & 30.5 & 48.2 & 48.6 & 45.4 & 41.7 \\
\cmidrule{2-18}
& SHOT \cite{shot}      & 28.0 & 30.1 & 28.8 & 25.0 & 26.0 & 38.0 & 45.7 & 51.0 & 51.5 & 59.1 & 70.6 & 30.2 & 48.4 & 47.8 & 45.8 & 41.7 \\
& TENT \cite{tent}      & 27.8 & 30.2 & 29.1 & 25.3 & 25.8 & 37.6 & 45.8 & 51.2 & 51.7 & 59.0 & 70.8 & 31.0 & 48.7 & 48.6 & 45.7 & 41.7 \\
& \gls{trust} naive            & 43.4 & 45.6 & 44.9 & 38.6 & 35.6 & 50.4 & 58.3 & 61.2 & 59.6 & 62.3 & 72.6 & 52.2 & 59.0 & 61.1 & 58.5 & 53.4 \\
& \ccol \gls{trust}            & \ccol \textbf{46.8} & \ccol \textbf{49.4} & \ccol \textbf{48.5} & \ccol \textbf{42.8} & \ccol \textbf{40.8} & \ccol \textbf{57.1} & \ccol \textbf{57.9} & \ccol \textbf{57.3} & \ccol \textbf{61.7} & \ccol \textbf{66.8} & \ccol \textbf{71.9} & \ccol \textbf{54.9} & \ccol \textbf{61.4} & \ccol \textbf{63.6} & \ccol \textbf{60.2} & \ccol \textbf{56.1} \\
\bottomrule
\end{tabular}
}
\caption{Top-1 classification accuracy under various corruption types on CIFAR10-C, CIFAR100-C, and ImageNet-C datasets.}
\label{main_online}
\end{table*}

\subsection{Implementation Details}
We perform adaptation exclusively on the Mamba-specific state space parameters within the \gls{ss2d} module of each VMamba block, while keeping the rest of the model frozen. Adaptation is guided using a pseudo-labeling strategy, where confident model predictions are treated as supervision targets in a cross-entropy loss. This enables self-supervised adaptation without requiring access to ground-truth labels. To stabilize training, we retain only high-confidence predictions as targets and discard uncertain ones. The adaptation proceeds in an online manner, with model updates applied sequentially. Optimization is performed using the Adam optimizer with a learning rate of $10^{-4}$ and a batch size of $128$, ensuring consistent dynamics and fair comparison across benchmarks. All experiments were conducted using a single NVIDIA $A6000$ GPU.

\subsection{Baselines}
We evaluate our method against several state-of-the-art \gls{tta} approaches: Source Only denotes the performance of VMamba without adaptation. ETA minimizes an entropy loss weighted by a sample-adaptive score and updates only the affine parameters of normalization layers.LAME enforces smooth decision boundaries through a Laplacian regularization objective. SAR promotes robustness by optimizing for flat minima using sharpness-aware minimization. SHOT aligns the classifier by minimizing entropy and promoting confident, diverse predictions. TENT adapts the model by updating only the affine parameters of normalization layers via entropy minimization. We evaluate two variants of our approach: \gls{trust} naive, which adapts only the Mamba-specific \gls{ss2d} parameters, and \gls{trust}, which further enhances robustness by averaging over traversal permutations.

\subsection{Main Results}
% We compare our method against several state-of-the-art \gls{tta} approaches, including \textit{Source Only} (VMamba without adaptation), ETA, LAME, SAR, SHOT, and TENT. We evaluate two variants of our approach: \gls{trust} naive, which adapts only the Mamba-specific \gls{ss2d} parameters, and \gls{trust}, which further enhances robustness via traversal-based prediction averaging. Table~\ref{main_online} presents Top-1 accuracy under the highest corruption severity for CIFAR10-C, CIFAR100-C, and ImageNet-C. \gls{trust} consistently surpasses all baselines, including its naive variant, demonstrating strong robustness under severe distribution shifts and validating the effectiveness of our adaptation strategy.

Table~\ref{main} presents the Top-1 accuracy under the highest corruption severity (level 5) for CIFAR10-C, CIFAR100-C, and ImageNet-C. \gls{trust} consistently outperforms all baselines across the three datasets, demonstrating strong generalization under severe distribution shifts. In addition, we also evaluate \textit{\gls{trust} naive}, which only adapts the Mamba-specific \gls{ss2d} parameters without applying traversal permutation. While \textit{\gls{trust} naive} provides a competitive and efficient performance over the other baselines, \gls{trust} delivers consistent improvements, underscoring the effectiveness of permutation-based adaptation for enhancing robustness.

\mypar{CIFAR10-C.} \gls{trust} achieves a mean accuracy of $77.5\%$, outperforming both TENT and SHOT by margins of $+11.0\%$ and $+11.2\%$, respectively. Compared to its naive variant, our full approach provides a further $+2.3\%$ boost. These results highlight the benefits of traversal diversity in enhancing corruption robustness. Notably, the gains are consistent across all corruption types, especially in elastic ($+7.9\%$) and fog ($+5.7\%$) conditions.

\mypar{CIFAR100-C.} On a more fine-grained benchmark, \gls{trust} attains a mean accuracy of $53.4\%$, exceeding TENT and SAR by $+9.7\%$ and $+12.4\%$, respectively. It also improves upon TRUST naive by $+2.5\%$. The largest absolute improvements are observed under challenging corruptions like frost ($+6.7\%$) and elastic ($+7.5\%$), demonstrating the method’s ability to generalize under severe distribution shifts.

\mypar{ImageNet-C.} \gls{trust} achieves a strong mean accuracy of $56.1\%$ on the large-scale ImageNet-C benchmark, outperforming both TENT and SHOT by $+14.4\%$, and TRUST naive by $+4.1\%$. The most notable gains appear under corruptions involving blur (e.g., motion blur: $+6.8\%$) and digital artifacts (e.g., jpeg compression: $+5.0\%$, contrast: $+4.5\%$), reflecting the advantage of our method in mitigating content distortion and noise.

In addition to corruption-specific robustness, our method demonstrates strong generalization to broader distribution shifts, as summarized in Table~\ref{domain_shift_online}. On \textbf{ImageNet-S}, our approach achieves $41.5\%$ accuracy, outperforming SHOT by a substantial $+8.9\%$ margin. For \textbf{ImageNet-V2}, \gls{trust} attains $64.0\%$, exceeding SHOT by $+1.6\%$ and providing a $+0.6\%$ gain over its naive variant. The most significant boost is observed on the \textbf{ImageNet-R} benchmark, which features real-world renditions of ImageNet categories. Here, our method achieves $44.3\%$, surpassing both TENT and SHOT by $+12.4\%$, and outperforming TRUST naive by $+4.6\%$. On the \textbf{PACS} dataset, our model reaches $69.9\%$ accuracy, offering consistent improvements over SHOT and TENT by $+2.5\%$, and over the naive variant by $+2.8\%$. These consistent gains across varied benchmarks highlight the adaptability of our permutation-based strategy, which not only improves corruption robustness but also scales effectively to domain generalization tasks.


\begin{table*}[htbp]
\setlength\tabcolsep{4pt}
\centering
\resizebox{0.9\textwidth}{!}{
\small
\begin{tabular}{l|ccccccc}
\toprule
\textbf{Method} & CIFAR10-C & CIFAR100-C & ImageNet-C & ImageNet-S & ImageNet-V2 & ImageNet-R & PACS \\
\midrule
Source only           & 65.9 & 41.2 & 38.7 & 31.4 & 62.2 & 31.3 & 66.7 \\
ETA \cite{eta}        & 65.8 & 41.4 & 40.8 & 31.4 & 62.2 & 31.3 & 66.7 \\
LAME \cite{lame}      & 65.9 & 41.2 & 38.8 & 31.4 & 62.2 & 31.3 & 66.7 \\
SAR \cite{sar}        & 66.8 & 41.9 & 41.5 & 32.6 & 62.4 & 32.0 & 67.3 \\
\cmidrule{1-8}
SHOT \cite{shot}      & 66.8 & 42.0 & 41.7 & 32.6 & 62.4 & 31.9 & 67.4 \\
TENT \cite{tent}      & 66.5 & 41.8 & 41.7 & 32.5 & 62.3 & 31.9 & 67.4 \\
\gls{trust} naive            & 74.2 & 49.8 & 53.4 & 41.1 & 63.4 & 39.7 & 67.1 \\
\ccol \gls{trust}            & \ccol \textbf{77.5} & \ccol \textbf{54.3} & \ccol \textbf{56.1} & \ccol \textbf{41.5} & \ccol \textbf{64.0} & \ccol \textbf{44.3} & \ccol \textbf{69.9} \\
\bottomrule
\end{tabular}
}
\caption{Average test-time adaptation performance (accuracy \%) across multiple datasets. For CIFAR10-C, CIFAR100-C, and ImageNet-C, the values represent the mean across all corruption types and severities. For ImageNet-S, ImageNet-V2, ImageNet-R, and PACS, the values correspond to classification accuracy on their respective test sets.}
\label{domain_shift_online}
\end{table*}


\subsection{Ablation Study}
In this section, we present a comprehensive ablation study on the CIFAR10-C dataset to assess the impact of key factors on our model’s performance. Specifically, we analyze the effects of batch size, augmentation types, number of traversal permutations, aggregation strategies, number of adaptation iterations, and computational overhead.

\mypar{Batch Size.} Figure~\ref{batch_size} demonstrates that \gls{trust} maintains a consistent advantage over TENT across all batch sizes. Even at smaller sizes such as 16 and 32, it delivers an accuracy improvement of around $8\%$. This indicates that our approach remains reliable and effective, even when operating with limited data per batch.

\mypar{Augmentation Impact.}
To evaluate whether standard data augmentations can serve as effective alternatives to our traversal permutation strategy, we compare \gls{trust} against common augmentations including rotation, random cropping, and color jitter. As shown in Figure~\ref{augmentation}, these traditional augmentations yield only modest improvements over the baseline source-only model on CIFAR10-C, with accuracies ranging from 65.9\% to 68.3\%. In contrast, our method achieves a substantial performance boost, reaching 77.5\%, which is significantly higher than all augmentation baselines. This indicates that simple augmentations fail to sufficiently address distribution shifts.

\begin{figure}[h]
  \centering
  \begin{minipage}[h]{0.48\textwidth}
    \includegraphics[width=\linewidth]{images/batch_size_CIFAR10.pdf}
    \vspace{-10pt}
    \caption{Accuracy comparison between \gls{trust} and TENT across varying batch sizes on CIFAR10-C dataset.}
    \label{batch_size}
  \end{minipage}\hfill
  \begin{minipage}[h]{0.48\textwidth}
    \includegraphics[width=\linewidth]{images/augmentation_10.pdf}
    \vspace{-10pt}
    \caption{Performance comparison between standard augmentations and \gls{trust} on CIFAR10-C dataset.}
    \label{augmentation}
  \end{minipage}
\end{figure}

\mypar{Number of Traversal Permutations.} We evaluate how the number of traversal permutations influences model accuracy across datasets (Figure~\ref{variation}). We observe a consistent performance improvement as the number of traversal permutations increases. On ImageNet-C, accuracy rises from 54.4\% with two permutations to 56.1\% with six. Similar trends are observed for CIFAR100-C (51.7\% to 54.3\%) and CIFAR10-C (75.6\% to 77.5\%), demonstrating that aggregating predictions from diverse traversal orders enhances robustness under distribution shifts. We select six permutations as a balanced choice between performance gains and computational cost. While accuracy continues to improve up to six, the marginal benefit begins to plateau beyond four permutations. Using six allows us to capture a broad set of complementary spatial perspectives without incurring excessive overhead. For further information about computational cost, refer to Figure~\ref{cc}.

\mypar{Number of Adaptation Iterations.} Figure~\ref{iteration} illustrates that accuracy improves progressively with an increasing number of iterations. Both our method and TENT benefit from additional iterations; however, our approach consistently achieves higher accuracy at every step. The performance gap is evident from the very first iteration and remains stable throughout, with our method outperforming TENT at all levels. Despite the potential for further improvement with more iterations, we chose to use only a single iteration in subsequent experiments to enable faster adaptation without compromising on competitive performance. All results in this experiment were obtained using a batch size of 128.

\begin{figure}[h]
  \centering
  \begin{minipage}[h]{0.48\textwidth}
    \includegraphics[width=\linewidth]{images/variation.pdf}
    \vspace{-10pt}
    \caption{Effect of traversal permutation count on accuracy across three datasets.}
    \label{variation}
  \end{minipage}\hfill
  \begin{minipage}[h]{0.48\textwidth}
    \includegraphics[width=\linewidth]{images/iteration.pdf}
    \vspace{-10pt}
    \caption{Model performance across adaptation iterations on CIFAR10-C dataset.}
    \label{iteration}
  \end{minipage}
\end{figure}

\mypar{Aggregation Strategy.} We evaluate two baseline strategies for aggregation across traversal permutations: (1) an ensemble approach that averages model predictions from independently processed traversal orders, and (2) a repetition baseline, where the same traversal permutation is applied $k$ times, followed by weight averaging. As shown in Figure~\ref{aggregation}, both baselines yield lower performance on CIFAR10-C, with ensemble achieving 68.1\% and repeating 69.6\%, compared to 75.6\% with our method. The ensemble captures traversal diversity but lacks the parameter alignment in our method, while the repetition baseline tests if gains come from sequential updates alone. Their lower performance shows our method works not just due to averaging, but because it strategically selects diverse traversal permutations that expose the model to varied contextual patterns, enhancing generalization under distribution shifts.

\mypar{Effect of Traversal Permutation in Evaluation.} Figure~\ref{eval} shows how accuracy varies depending on the traversal permutation used during evaluation. We observe that different traversal permutation lead to noticeably different performance levels. The default permutation used in the original VMamba architecture, "abcd", achieves the highest accuracy at 77.5\%. Other permutations, such as "badc", perform significantly worse (e.g., 71.6\%), indicating that the choice of evaluation traversal can substantially impact the model’s output. Due to this sensitivity, we adopt the abcd order for evaluation in all our experiments to maintain consistency and leverage the strongest baseline.

\begin{figure}[h]
  \centering
  \begin{minipage}[h]{0.48\textwidth}
    \includegraphics[width=\linewidth]{images/aggregation.pdf}
    \vspace{-10pt}
    \caption{Accuracy comparison of different aggregation strategies on CIFAR10-C dataset.}
    \label{aggregation}
  \end{minipage}\hfill
  \begin{minipage}[h]{0.48\textwidth}
    \includegraphics[width=\linewidth]{images/eval.pdf}
    \vspace{-10pt}
    \caption{Impact of traversal permutation during evaluation on CIFAR10-C dataset.}
    \label{eval}
  \end{minipage}
\end{figure}

\begin{wrapfigure}{r}{0.48\textwidth}
  \vspace{-10pt}
  \centering
  \includegraphics[width=\linewidth]{images/cc.pdf}
  \vspace{-10pt}
  \caption{GPU memory usage increases with the number of traversals. The baseline memory is 0.998 GB for a single traversal, and usage increases proportionally with more traversals.}
  \label{cc}
\end{wrapfigure}

\mypar{Computational Overhead.} \lipsum[1]

==> Backup/sec/7_checklist.tex <==
\section*{NeurIPS Paper Checklist}

%%% BEGIN INSTRUCTIONS %%%
The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
limit. 

Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
\begin{itemize}
    \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
    \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
    \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
   % \item {\bf The papers not including the checklist will be desk rejected.}
\end{itemize}

{\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

IMPORTANT, please:
\begin{itemize}
    \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
    \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
    \item {\bf Do not modify the questions and only use the provided macros for your answers}.
\end{itemize} 
 

%%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: Yes, the abstract is summary of the content of the paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerTODO{} % Replace by \answerYes{}, \answerNo{}, or \answerNA{}.
    \item[] Justification: \justificationTODO{}
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}

==> sec/7_checklist.tex <==
\section*{NeurIPS Paper Checklist}

% %%% BEGIN INSTRUCTIONS %%%
% The checklist is designed to encourage best practices for responsible machine learning research, addressing issues of reproducibility, transparency, research ethics, and societal impact. Do not remove the checklist: {\bf The papers not including the checklist will be desk rejected.} The checklist should follow the references and follow the (optional) supplemental material.  The checklist does NOT count towards the page
% limit. 

% Please read the checklist guidelines carefully for information on how to answer these questions. For each question in the checklist:
% \begin{itemize}
%     \item You should answer \answerYes{}, \answerNo{}, or \answerNA{}.
%     \item \answerNA{} means either that the question is Not Applicable for that particular paper or the relevant information is Not Available.
%     \item Please provide a short (1–2 sentence) justification right after your answer (even for NA). 
%    % \item {\bf The papers not including the checklist will be desk rejected.}
% \end{itemize}

% {\bf The checklist answers are an integral part of your paper submission.} They are visible to the reviewers, area chairs, senior area chairs, and ethics reviewers. You will be asked to also include it (after eventual revisions) with the final version of your paper, and its final version will be published with the paper.

% The reviewers of your paper will be asked to use the checklist as one of the factors in their evaluation. While "\answerYes{}" is generally preferable to "\answerNo{}", it is perfectly acceptable to answer "\answerNo{}" provided a proper justification is given (e.g., "error bars are not reported because it would be too computationally expensive" or "we were unable to find the license for the dataset we used"). In general, answering "\answerNo{}" or "\answerNA{}" is not grounds for rejection. While the questions are phrased in a binary way, we acknowledge that the true answer is often more nuanced, so please just use your best judgment and write a justification to elaborate. All supporting evidence can appear either in the main paper or the supplemental material, provided in appendix. If you answer \answerYes{} to a question, in the justification please point to the section(s) where related material for the question can be found.

% IMPORTANT, please:
% \begin{itemize}
%     \item {\bf Delete this instruction block, but keep the section heading ``NeurIPS Paper Checklist"},
%     \item  {\bf Keep the checklist subsection headings, questions/answers and guidelines below.}
%     \item {\bf Do not modify the questions and only use the provided macros for your answers}.
% \end{itemize} 
 

% %%% END INSTRUCTIONS %%%


\begin{enumerate}

\item {\bf Claims}
    \item[] Question: Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \item[] Answer: \answerYes{}
    \item[] Justification: The abstract is the summary of the content of the paper and the introduction is clearly state the main contributions of the paper.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the abstract and introduction do not include the claims made in the paper.
        \item The abstract and/or introduction should clearly state the claims made, including the contributions made in the paper and important assumptions and limitations. A No or NA answer to this question will not be perceived well by the reviewers. 
        \item The claims made should match theoretical and experimental results, and reflect how much the results can be expected to generalize to other settings. 
        \item It is fine to include aspirational goals as motivation as long as it is clear that these goals are not attained by the paper. 
    \end{itemize}

\item {\bf Limitations}
    \item[] Question: Does the paper discuss the limitations of the work performed by the authors?
    \item[] Answer: \answerYes{}
    \item[] Justification: In the last part of the conclusion section.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper has no limitation while the answer No means that the paper has limitations, but those are not discussed in the paper. 
        \item The authors are encouraged to create a separate "Limitations" section in their paper.
        \item The paper should point out any strong assumptions and how robust the results are to violations of these assumptions (e.g., independence assumptions, noiseless settings, model well-specification, asymptotic approximations only holding locally). The authors should reflect on how these assumptions might be violated in practice and what the implications would be.
        \item The authors should reflect on the scope of the claims made, e.g., if the approach was only tested on a few datasets or with a few runs. In general, empirical results often depend on implicit assumptions, which should be articulated.
        \item The authors should reflect on the factors that influence the performance of the approach. For example, a facial recognition algorithm may perform poorly when image resolution is low or images are taken in low lighting. Or a speech-to-text system might not be used reliably to provide closed captions for online lectures because it fails to handle technical jargon.
        \item The authors should discuss the computational efficiency of the proposed algorithms and how they scale with dataset size.
        \item If applicable, the authors should discuss possible limitations of their approach to address problems of privacy and fairness.
        \item While the authors might fear that complete honesty about limitations might be used by reviewers as grounds for rejection, a worse outcome might be that reviewers discover limitations that aren't acknowledged in the paper. The authors should use their best judgment and recognize that individual actions in favor of transparency play an important role in developing norms that preserve the integrity of the community. Reviewers will be specifically instructed to not penalize honesty concerning limitations.
    \end{itemize}

\item {\bf Theory assumptions and proofs}
    \item[] Question: For each theoretical result, does the paper provide the full set of assumptions and a complete (and correct) proof?
    \item[] Answer: \answerNA{}
    \item[] Justification: No theoretical results.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include theoretical results. 
        \item All the theorems, formulas, and proofs in the paper should be numbered and cross-referenced.
        \item All assumptions should be clearly stated or referenced in the statement of any theorems.
        \item The proofs can either appear in the main paper or the supplemental material, but if they appear in the supplemental material, the authors are encouraged to provide a short proof sketch to provide intuition. 
        \item Inversely, any informal proof provided in the core of the paper should be complemented by formal proofs provided in appendix or supplemental material.
        \item Theorems and Lemmas that the proof relies upon should be properly referenced. 
    \end{itemize}

    \item {\bf Experimental result reproducibility}
    \item[] Question: Does the paper fully disclose all the information needed to reproduce the main experimental results of the paper to the extent that it affects the main claims and/or conclusions of the paper (regardless of whether the code and data are provided or not)?
    \item[] Answer: \answerYes{}
    \item[] Justification: We provide details of implementation and experiments in section 4.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item If the paper includes experiments, a No answer to this question will not be perceived well by the reviewers: Making the paper reproducible is important, regardless of whether the code and data are provided or not.
        \item If the contribution is a dataset and/or model, the authors should describe the steps taken to make their results reproducible or verifiable. 
        \item Depending on the contribution, reproducibility can be accomplished in various ways. For example, if the contribution is a novel architecture, describing the architecture fully might suffice, or if the contribution is a specific model and empirical evaluation, it may be necessary to either make it possible for others to replicate the model with the same dataset, or provide access to the model. In general. releasing code and data is often one good way to accomplish this, but reproducibility can also be provided via detailed instructions for how to replicate the results, access to a hosted model (e.g., in the case of a large language model), releasing of a model checkpoint, or other means that are appropriate to the research performed.
        \item While NeurIPS does not require releasing code, the conference does require all submissions to provide some reasonable avenue for reproducibility, which may depend on the nature of the contribution. For example
        \begin{enumerate}
            \item If the contribution is primarily a new algorithm, the paper should make it clear how to reproduce that algorithm.
            \item If the contribution is primarily a new model architecture, the paper should describe the architecture clearly and fully.
            \item If the contribution is a new model (e.g., a large language model), then there should either be a way to access this model for reproducing the results or a way to reproduce the model (e.g., with an open-source dataset or instructions for how to construct the dataset).
            \item We recognize that reproducibility may be tricky in some cases, in which case authors are welcome to describe the particular way they provide for reproducibility. In the case of closed-source models, it may be that access to the model is limited in some way (e.g., to registered users), but it should be possible for other researchers to have some path to reproducing or verifying the results.
        \end{enumerate}
    \end{itemize}


\item {\bf Open access to data and code}
    \item[] Question: Does the paper provide open access to the data and code, with sufficient instructions to faithfully reproduce the main experimental results, as described in supplemental material?
    \item[] Answer: \answerYes{}
    \item[] Justification: The data is available online and we will release the code with the supplementary material.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that paper does not include experiments requiring code.
        \item Please see the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item While we encourage the release of code and data, we understand that this might not be possible, so “No” is an acceptable answer. Papers cannot be rejected simply for not including code, unless this is central to the contribution (e.g., for a new open-source benchmark).
        \item The instructions should contain the exact command and environment needed to run to reproduce the results. See the NeurIPS code and data submission guidelines (\url{https://nips.cc/public/guides/CodeSubmissionPolicy}) for more details.
        \item The authors should provide instructions on data access and preparation, including how to access the raw data, preprocessed data, intermediate data, and generated data, etc.
        \item The authors should provide scripts to reproduce all experimental results for the new proposed method and baselines. If only a subset of experiments are reproducible, they should state which ones are omitted from the script and why.
        \item At submission time, to preserve anonymity, the authors should release anonymized versions (if applicable).
        \item Providing as much information as possible in supplemental material (appended to the paper) is recommended, but including URLs to data and code is permitted.
    \end{itemize}


\item {\bf Experimental setting/details}
    \item[] Question: Does the paper specify all the training and test details (e.g., data splits, hyperparameters, how they were chosen, type of optimizer, etc.) necessary to understand the results?
    \item[] Answer: \answerYes{}
    \item[] Justification: Provided in section 4.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The experimental setting should be presented in the core of the paper to a level of detail that is necessary to appreciate the results and make sense of them.
        \item The full details can be provided either with the code, in appendix, or as supplemental material.
    \end{itemize}

\item {\bf Experiment statistical significance}
    \item[] Question: Does the paper report error bars suitably and correctly defined or other appropriate information about the statistical significance of the experiments?
    \item[] Answer: \answerNo{}
    \item[] Justification: Experiments were run with a single seed. We plan to include multi-seed results in future revisions.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The authors should answer "Yes" if the results are accompanied by error bars, confidence intervals, or statistical significance tests, at least for the experiments that support the main claims of the paper.
        \item The factors of variability that the error bars are capturing should be clearly stated (for example, train/test split, initialization, random drawing of some parameter, or overall run with given experimental conditions).
        \item The method for calculating the error bars should be explained (closed form formula, call to a library function, bootstrap, etc.)
        \item The assumptions made should be given (e.g., Normally distributed errors).
        \item It should be clear whether the error bar is the standard deviation or the standard error of the mean.
        \item It is OK to report 1-sigma error bars, but one should state it. The authors should preferably report a 2-sigma error bar than state that they have a 96\% CI, if the hypothesis of Normality of errors is not verified.
        \item For asymmetric distributions, the authors should be careful not to show in tables or figures symmetric error bars that would yield results that are out of range (e.g. negative error rates).
        \item If error bars are reported in tables or plots, The authors should explain in the text how they were calculated and reference the corresponding figures or tables in the text.
    \end{itemize}

\item {\bf Experiments compute resources}
    \item[] Question: For each experiment, does the paper provide sufficient information on the computer resources (type of compute workers, memory, time of execution) needed to reproduce the experiments?
    \item[] Answer: \answerYes{}
    \item[] Justification: The paper provides details on the hardware used, and reports a computational overhead analysis in the ablation section.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not include experiments.
        \item The paper should indicate the type of compute workers CPU or GPU, internal cluster, or cloud provider, including relevant memory and storage.
        \item The paper should provide the amount of compute required for each of the individual experimental runs as well as estimate the total compute. 
        \item The paper should disclose whether the full research project required more compute than the experiments reported in the paper (e.g., preliminary or failed experiments that didn't make it into the paper). 
    \end{itemize}
    
\item {\bf Code of ethics}
    \item[] Question: Does the research conducted in the paper conform, in every respect, with the NeurIPS Code of Ethics \url{https://neurips.cc/public/EthicsGuidelines}?
    \item[] Answer: \answerYes{}
    \item[] Justification: Yes, we do.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the authors have not reviewed the NeurIPS Code of Ethics.
        \item If the authors answer No, they should explain the special circumstances that require a deviation from the Code of Ethics.
        \item The authors should make sure to preserve anonymity (e.g., if there is a special consideration due to laws or regulations in their jurisdiction).
    \end{itemize}


\item {\bf Broader impacts}
    \item[] Question: Does the paper discuss both potential positive societal impacts and negative societal impacts of the work performed?
    \item[] Answer: \answerNA{}
    \item[] Justification: No relevant.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that there is no societal impact of the work performed.
        \item If the authors answer NA or No, they should explain why their work has no societal impact or why the paper does not address societal impact.
        \item Examples of negative societal impacts include potential malicious or unintended uses (e.g., disinformation, generating fake profiles, surveillance), fairness considerations (e.g., deployment of technologies that could make decisions that unfairly impact specific groups), privacy considerations, and security considerations.
        \item The conference expects that many papers will be foundational research and not tied to particular applications, let alone deployments. However, if there is a direct path to any negative applications, the authors should point it out. For example, it is legitimate to point out that an improvement in the quality of generative models could be used to generate deepfakes for disinformation. On the other hand, it is not needed to point out that a generic algorithm for optimizing neural networks could enable people to train models that generate Deepfakes faster.
        \item The authors should consider possible harms that could arise when the technology is being used as intended and functioning correctly, harms that could arise when the technology is being used as intended but gives incorrect results, and harms following from (intentional or unintentional) misuse of the technology.
        \item If there are negative societal impacts, the authors could also discuss possible mitigation strategies (e.g., gated release of models, providing defenses in addition to attacks, mechanisms for monitoring misuse, mechanisms to monitor how a system learns from feedback over time, improving the efficiency and accessibility of ML).
    \end{itemize}
    
\item {\bf Safeguards}
    \item[] Question: Does the paper describe safeguards that have been put in place for responsible release of data or models that have a high risk for misuse (e.g., pretrained language models, image generators, or scraped datasets)?
    \item[] Answer: \answerNA{}
    \item[] Justification: No relevant.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper poses no such risks.
        \item Released models that have a high risk for misuse or dual-use should be released with necessary safeguards to allow for controlled use of the model, for example by requiring that users adhere to usage guidelines or restrictions to access the model or implementing safety filters. 
        \item Datasets that have been scraped from the Internet could pose safety risks. The authors should describe how they avoided releasing unsafe images.
        \item We recognize that providing effective safeguards is challenging, and many papers do not require this, but we encourage authors to take this into account and make a best faith effort.
    \end{itemize}

\item {\bf Licenses for existing assets}
    \item[] Question: Are the creators or original owners of assets (e.g., code, data, models), used in the paper, properly credited and are the license and terms of use explicitly mentioned and properly respected?
    \item[] Answer: \answerYes{}
    \item[] Justification: We followed the protocol.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not use existing assets.
        \item The authors should cite the original paper that produced the code package or dataset.
        \item The authors should state which version of the asset is used and, if possible, include a URL.
        \item The name of the license (e.g., CC-BY 4.0) should be included for each asset.
        \item For scraped data from a particular source (e.g., website), the copyright and terms of service of that source should be provided.
        \item If assets are released, the license, copyright information, and terms of use in the package should be provided. For popular datasets, \url{paperswithcode.com/datasets} has curated licenses for some datasets. Their licensing guide can help determine the license of a dataset.
        \item For existing datasets that are re-packaged, both the original license and the license of the derived asset (if it has changed) should be provided.
        \item If this information is not available online, the authors are encouraged to reach out to the asset's creators.
    \end{itemize}

\item {\bf New assets}
    \item[] Question: Are new assets introduced in the paper well documented and is the documentation provided alongside the assets?
    \item[] Answer: \answerNo{}
    \item[] Justification: The paper does not introduce any new datasets or benchmarks. All experiments are conducted on existing public datasets using open-source baselines.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not release new assets.
        \item Researchers should communicate the details of the dataset/code/model as part of their submissions via structured templates. This includes details about training, license, limitations, etc. 
        \item The paper should discuss whether and how consent was obtained from people whose asset is used.
        \item At submission time, remember to anonymize your assets (if applicable). You can either create an anonymized URL or include an anonymized zip file.
    \end{itemize}

\item {\bf Crowdsourcing and research with human subjects}
    \item[] Question: For crowdsourcing experiments and research with human subjects, does the paper include the full text of instructions given to participants and screenshots, if applicable, as well as details about compensation (if any)? 
    \item[] Answer: \answerNA{}
    \item[] Justification: The paper does not involve crowdsourcing experiments or research with human subjects.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Including this information in the supplemental material is fine, but if the main contribution of the paper involves human subjects, then as much detail as possible should be included in the main paper. 
        \item According to the NeurIPS Code of Ethics, workers involved in data collection, curation, or other labor should be paid at least the minimum wage in the country of the data collector. 
    \end{itemize}

\item {\bf Institutional review board (IRB) approvals or equivalent for research with human subjects}
    \item[] Question: Does the paper describe potential risks incurred by study participants, whether such risks were disclosed to the subjects, and whether Institutional Review Board (IRB) approvals (or an equivalent approval/review based on the requirements of your country or institution) were obtained?
    \item[] Answer: \answerNA{}
    \item[] Justification: Not relevant.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the paper does not involve crowdsourcing nor research with human subjects.
        \item Depending on the country in which research is conducted, IRB approval (or equivalent) may be required for any human subjects research. If you obtained IRB approval, you should clearly state this in the paper. 
        \item We recognize that the procedures for this may vary significantly between institutions and locations, and we expect authors to adhere to the NeurIPS Code of Ethics and the guidelines for their institution. 
        \item For initial submissions, do not include any information that would break anonymity (if applicable), such as the institution conducting the review.
    \end{itemize}

\item {\bf Declaration of LLM usage}
    \item[] Question: Does the paper describe the usage of LLMs if it is an important, original, or non-standard component of the core methods in this research? Note that if the LLM is used only for writing, editing, or formatting purposes and does not impact the core methodology, scientific rigorousness, or originality of the research, declaration is not required.
    %this research? 
    \item[] Answer: \answerNo{}
    \item[] Justification: This work does not use LLMs in the core methodology, scientific rigorousness, or originality of the research.
    \item[] Guidelines:
    \begin{itemize}
        \item The answer NA means that the core method development in this research does not involve LLMs as any important, original, or non-standard components.
        \item Please refer to our LLM policy (\url{https://neurips.cc/Conferences/2025/LLM}) for what should or should not be described.
    \end{itemize}

\end{enumerate}
